Padding to k: A Minimum Count in the Schema Makes Open-Weight Models Pad Their Extraction Lists

Extraction pipelines ask language models for JSON that follows a schema, and the schema can set a minimum number of list entries. We ask what models do when the document holds fewer items than that minimum. Under a preregistered plan, we test eight open-weight models on 558 real documents from nine annotated datasets, with six more models on hosted services as a reference. Three findings stand out. First, models treat the count as a target: a minimum shown in the schema, but not enforced, raises the share of lists longer than the true count from 34.5% to 55.4%. Second, the padding is hard to catch, because most added entries are real text taken from the document; about half of them pass a check that each entry occurs in the source. Third, common fixes help only partly: a line saying fewer items are fine removes the effect on average but misses more true items, a count in prose ("up to k") also raises over-counting, an "N/A" option under an enforced minimum still leaves half the lists padded, and re-asking with the validation error makes padding far more common. We release the code, answer lists and run records at https://github.com/AbhishekBarali/padding-to-k

==> generated/app_named_per_model_rows.tex <==
  Qwen3.5-0.8B & +0.03 [$-$0.39, +0.47] & +0.62 [+0.19, +1.05] & $-$0.27 [$-$0.64, +0.09] & $-$0.25 [$-$0.60, +0.11] & +0.44 [$-$0.38, +1.29] & $-$1.0 [$-$3.8, +1.9] \\
  Qwen3.5-2B & $-$2.70 [$-$3.91, $-$1.56] & $-$3.31 [$-$4.26, $-$2.35] & $-$1.52 [$-$2.37, $-$0.70] & $-$0.43 [$-$1.46, +0.52] & +0.55 [$-$1.42, +2.58] & +1.9 [+0.0, +4.8] \\
  Qwen3.5-9B & $-$0.58 [$-$0.70, $-$0.46] & $-$1.20 [$-$1.34, $-$1.06] & $-$0.19 [$-$0.27, $-$0.10] & $-$0.00 [$-$0.13, +0.12] & +0.72 [+0.33, +1.03] & +6.7 [+2.9, +11.4] \\
  Qwen3.5-27B & +0.46 [+0.37, +0.56] & $-$0.78 [$-$0.88, $-$0.68] & $-$0.05 [$-$0.12, +0.02] & $-$0.09 [$-$0.16, $-$0.03] & +1.52 [+1.31, +1.75] & +7.6 [+2.9, +12.4] \\
  Gemma 4 31B & +0.02 [$-$0.02, +0.06] & $-$1.65 [$-$1.79, $-$1.52] & $-$0.02 [$-$0.05, +0.01] & +0.08 [+0.05, +0.12] & +1.48 [+1.34, +1.63] & +15.2 [+9.5, +21.0] \\
  Olmo 3.1 32B & $-$1.92 [$-$2.20, $-$1.66] & $-$2.18 [$-$2.43, $-$1.95] & $-$0.94 [$-$1.19, $-$0.70] & $-$0.24 [$-$0.37, $-$0.12] & +0.89 [+0.63, +1.17] & +4.8 [$-$1.0, +10.5] \\
  Ministral 3 14B & $-$1.50 [$-$1.76, $-$1.25] & $-$1.80 [$-$1.99, $-$1.62] & $-$0.83 [$-$1.02, $-$0.65] & $-$0.32 [$-$0.45, $-$0.19] & +1.01 [+0.72, +1.32] & +3.8 [$-$1.0, +8.6] \\
  gpt-oss-20b & +0.06 [$-$0.08, +0.19] & $-$0.81 [$-$0.93, $-$0.69] & $-$0.11 [$-$0.26, +0.03] & +0.05 [$-$0.06, +0.17] & +0.80 [+0.54, +1.04] & +20.0 [+14.3, +25.7] \\


==> generated/app_outcomes_per_model_a_rows.tex <==
  Qwen3.5-0.8B & \cnd{none} & 909 & 30.9 & 30.9 & 3.45 & 54.2 & 19.7 & 1.8 & 24.3 & 9.5 & 66.7 \\
  Qwen3.5-0.8B & \cnd{prose\_up\_to\_k} & 4545 & 50.0 & 49.8 & 2.75 & 28.0 & 32.5 & 20.2 & 19.4 & 16.3 & 53.5 \\
  Qwen3.5-0.8B & \cnd{prose\_exactly\_k} & 4545 & 39.6 & 39.4 & 2.35 & 45.0 & 21.0 & 18.6 & 15.3 & 11.8 & 65.1 \\
  Qwen3.5-0.8B & \cnd{max\_k\_shown} & 909 & 29.3 & 29.2 & 3.21 & 57.5 & 18.0 & 2.2 & 22.2 & 9.6 & 68.8 \\
  Qwen3.5-0.8B & \cnd{min\_k\_shown} & 909 & 24.9 & 24.9 & 3.02 & 67.4 & 11.6 & 2.4 & 18.6 & 5.6 & 76.5 \\
  Qwen3.5-0.8B & \cnd{min\_k\_shown\_fewer\_ok} & 909 & 34.0 & 33.9 & 3.42 & 49.1 & 21.2 & 3.7 & 26.0 & 12.9 & 65.1 \\
  Qwen3.5-0.8B & \cnd{min\_k\_enforced} & 909 & 91.9 & 91.5 & 6.13 & 0.8 & 1.0 & 34.3 & 63.9 & 6.6 & 15.6 \\
  Qwen3.5-0.8B & \cnd{min\_k\_escape} & 908 & 89.6 & 89.1 & 5.32 & 1.0 & 0.8 & 35.0 & 63.2 & 7.9 & 15.1 \\
  Qwen3.5-2B & \cnd{none} & 909 & 55.1 & 55.0 & 8.97 & 0.1 & 56.8 & 5.9 & 37.2 & 38.3 & 15.1 \\
  Qwen3.5-2B & \cnd{prose\_up\_to\_k} & 4545 & 58.9 & 58.7 & 4.36 & 0.6 & 51.4 & 26.4 & 21.5 & 34.7 & 21.1 \\
  Qwen3.5-2B & \cnd{prose\_exactly\_k} & 4545 & 58.4 & 58.3 & 3.92 & 0.2 & 50.8 & 30.4 & 18.7 & 35.8 & 21.8 \\
  Qwen3.5-2B & \cnd{max\_k\_shown} & 909 & 55.7 & 55.3 & 7.45 & 0.1 & 55.7 & 9.4 & 34.9 & 37.3 & 17.5 \\
  Qwen3.5-2B & \cnd{min\_k\_shown} & 909 & 60.4 & 60.3 & 9.56 & 0.2 & 47.9 & 14.6 & 37.3 & 34.1 & 17.0 \\
  Qwen3.5-2B & \cnd{min\_k\_shown\_fewer\_ok} & 909 & 46.9 & 46.9 & 6.47 & 0.7 & 56.0 & 9.6 & 33.8 & 34.3 & 23.8 \\
  Qwen3.5-2B & \cnd{min\_k\_enforced} & 908 & 94.5 & 94.1 & 4.65 & 0.0 & 1.1 & 43.7 & 55.2 & 5.2 & 12.1 \\
  Qwen3.5-2B & \cnd{min\_k\_escape} & 907 & 83.0 & 82.8 & 3.99 & 0.1 & 0.8 & 48.8 & 50.3 & 13.9 & 13.6 \\
  Qwen3.5-9B & \cnd{none} & 909 & 26.3 & 26.1 & 0.98 & 0.0 & 84.4 & 5.2 & 10.5 & 61.5 & 13.5 \\
  Qwen3.5-9B & \cnd{prose\_up\_to\_k} & 4545 & 34.1 & 33.7 & 0.81 & 0.1 & 79.3 & 18.7 & 1.9 & 56.9 & 17.8 \\
  Qwen3.5-9B & \cnd{prose\_exactly\_k} & 4545 & 38.9 & 38.6 & 0.92 & 0.0 & 71.2 & 27.5 & 1.4 & 51.5 & 18.2 \\
  Qwen3.5-9B & \cnd{max\_k\_shown} & 909 & 28.9 & 28.5 & 0.79 & 0.0 & 84.0 & 11.6 & 4.4 & 58.7 & 16.6 \\
  Qwen3.5-9B & \cnd{min\_k\_shown} & 909 & 44.8 & 44.6 & 1.56 & 0.1 & 62.0 & 25.7 & 12.1 & 46.1 & 11.6 \\
  Qwen3.5-9B & \cnd{min\_k\_shown\_fewer\_ok} & 909 & 18.0 & 17.9 & 0.67 & 0.0 & 86.4 & 6.6 & 7.0 & 55.1 & 26.9 \\
  Qwen3.5-9B & \cnd{min\_k\_enforced} & 909 & 92.7 & 92.4 & 3.24 & 0.2 & 0.7 & 75.4 & 23.8 & 6.6 & 6.4 \\
  Qwen3.5-9B & \cnd{min\_k\_escape} & 909 & 47.2 & 46.9 & 1.40 & 0.0 & 0.0 & 87.5 & 12.5 & 40.2 & 13.2 \\
  Qwen3.5-27B & \cnd{none} & 909 & 23.1 & 23.1 & 0.52 & 0.0 & 88.6 & 5.8 & 5.6 & 71.0 & 5.2 \\
  Qwen3.5-27B & \cnd{prose\_up\_to\_k} & 4545 & 29.5 & 29.5 & 0.59 & 0.7 & 80.7 & 18.4 & 0.1 & 64.9 & 10.0 \\
  Qwen3.5-27B & \cnd{prose\_exactly\_k} & 4545 & 42.1 & 42.0 & 0.94 & 0.8 & 64.2 & 34.9 & 0.1 & 53.6 & 9.8 \\
  Qwen3.5-27B & \cnd{max\_k\_shown} & 909 & 26.4 & 26.3 & 0.46 & 0.0 & 85.9 & 14.1 & 0.0 & 68.6 & 9.5 \\
  Qwen3.5-27B & \cnd{min\_k\_shown} & 909 & 60.9 & 60.6 & 1.72 & 2.4 & 38.9 & 51.4 & 7.3 & 35.0 & 4.8 \\
  Qwen3.5-27B & \cnd{min\_k\_shown\_fewer\_ok} & 909 & 42.2 & 42.1 & 0.97 & 1.5 & 61.9 & 35.4 & 1.1 & 51.6 & 7.1 \\
  Qwen3.5-27B & \cnd{min\_k\_enforced} & 909 & 91.6 & 91.4 & 2.57 & 0.0 & 0.6 & 91.2 & 8.3 & 7.9 & 4.1 \\
  Qwen3.5-27B & \cnd{min\_k\_escape} & 909 & 43.6 & 43.1 & 0.97 & 0.0 & 0.1 & 97.2 & 2.6 & 53.8 & 6.2 \\


==> generated/app_outcomes_per_model_b_rows.tex <==
  Gemma 4 31B & \cnd{none} & 909 & 14.4 & 14.2 & 0.20 & 0.0 & 95.6 & 3.2 & 1.2 & 77.8 & 8.6 \\
  Gemma 4 31B & \cnd{prose\_up\_to\_k} & 4545 & 16.5 & 16.2 & 0.24 & 0.0 & 95.1 & 4.9 & 0.0 & 76.5 & 12.0 \\
  Gemma 4 31B & \cnd{prose\_exactly\_k} & 4545 & 50.9 & 50.5 & 1.12 & 0.9 & 56.3 & 42.8 & 0.0 & 46.4 & 9.8 \\
  Gemma 4 31B & \cnd{max\_k\_shown} & 909 & 13.6 & 13.4 & 0.18 & 0.0 & 95.4 & 4.5 & 0.1 & 79.0 & 12.0 \\
  Gemma 4 31B & \cnd{min\_k\_shown} & 909 & 62.5 & 62.4 & 1.82 & 4.0 & 38.2 & 44.8 & 13.1 & 33.4 & 5.2 \\
  Gemma 4 31B & \cnd{min\_k\_shown\_fewer\_ok} & 909 & 16.0 & 15.7 & 0.22 & 0.0 & 93.8 & 5.4 & 0.8 & 77.2 & 7.9 \\
  Gemma 4 31B & \cnd{min\_k\_enforced} & 909 & 85.6 & 85.3 & 2.38 & 0.0 & 0.1 & 86.7 & 13.2 & 13.5 & 4.2 \\
  Gemma 4 31B & \cnd{min\_k\_escape} & 909 & 29.9 & 29.9 & 0.62 & 0.0 & 0.0 & 96.6 & 3.4 & 62.9 & 7.3 \\
  Olmo 3.1 32B & \cnd{none} & 909 & 42.2 & 41.7 & 2.01 & 0.9 & 67.8 & 7.5 & 23.9 & 50.4 & 11.5 \\
  Olmo 3.1 32B & \cnd{prose\_up\_to\_k} & 4545 & 49.2 & 48.8 & 1.32 & 0.3 & 61.3 & 33.0 & 5.4 & 45.3 & 18.5 \\
  Olmo 3.1 32B & \cnd{prose\_exactly\_k} & 4545 & 54.8 & 54.4 & 1.34 & 0.4 & 51.6 & 46.3 & 1.7 & 39.2 & 20.2 \\
  Olmo 3.1 32B & \cnd{max\_k\_shown} & 909 & 45.0 & 44.7 & 1.07 & 0.9 & 64.4 & 31.7 & 3.1 & 47.4 & 18.4 \\
  Olmo 3.1 32B & \cnd{min\_k\_shown} & 909 & 57.8 & 57.4 & 2.25 & 1.3 & 44.2 & 37.4 & 17.1 & 35.9 & 12.9 \\
  Olmo 3.1 32B & \cnd{min\_k\_shown\_fewer\_ok} & 909 & 18.7 & 18.5 & 0.49 & 2.9 & 83.3 & 10.0 & 3.9 & 51.3 & 34.6 \\
  Olmo 3.1 32B & \cnd{min\_k\_enforced} & 909 & 95.6 & 93.0 & 3.65 & 0.0 & 0.6 & 73.2 & 26.3 & 4.2 & 9.1 \\
  Olmo 3.1 32B & \cnd{min\_k\_escape} & 909 & 49.5 & 49.3 & 1.90 & 0.0 & 0.0 & 80.5 & 19.5 & 41.9 & 15.3 \\
  Ministral 3 14B & \cnd{none} & 909 & 50.2 & 49.9 & 2.07 & 0.0 & 68.0 & 7.5 & 24.5 & 47.5 & 6.9 \\
  Ministral 3 14B & \cnd{prose\_up\_to\_k} & 4545 & 59.9 & 59.6 & 1.51 & 0.1 & 58.0 & 39.0 & 2.9 & 38.5 & 12.5 \\
  Ministral 3 14B & \cnd{prose\_exactly\_k} & 4545 & 67.5 & 67.1 & 1.70 & 0.2 & 45.4 & 52.9 & 1.5 & 31.2 & 12.7 \\
  Ministral 3 14B & \cnd{max\_k\_shown} & 909 & 46.5 & 46.5 & 1.25 & 0.0 & 70.0 & 21.5 & 8.6 & 50.6 & 10.3 \\
  Ministral 3 14B & \cnd{min\_k\_shown} & 909 & 67.7 & 67.2 & 2.35 & 0.0 & 42.1 & 40.4 & 17.5 & 31.8 & 8.1 \\
  Ministral 3 14B & \cnd{min\_k\_shown\_fewer\_ok} & 909 & 32.7 & 32.6 & 0.72 & 0.0 & 77.9 & 19.8 & 2.3 & 55.8 & 17.2 \\
  Ministral 3 14B & \cnd{min\_k\_enforced} & 909 & 97.2 & 96.9 & 3.14 & 0.3 & 0.3 & 82.2 & 17.2 & 2.2 & 9.9 \\
  Ministral 3 14B & \cnd{min\_k\_escape} & 909 & 24.3 & 24.2 & 0.60 & 0.0 & 0.0 & 93.6 & 6.4 & 49.6 & 29.4 \\
  gpt-oss-20b & \cnd{none} & 909 & 33.9 & 33.8 & 1.04 & 0.0 & 79.6 & 8.1 & 12.2 & 59.7 & 8.6 \\
  gpt-oss-20b & \cnd{prose\_up\_to\_k} & 4545 & 43.7 & 43.2 & 1.08 & 0.0 & 66.3 & 31.7 & 1.9 & 52.1 & 14.5 \\
  gpt-oss-20b & \cnd{prose\_exactly\_k} & 4545 & 54.9 & 54.5 & 1.36 & 0.3 & 40.6 & 58.5 & 0.7 & 41.2 & 15.0 \\
  gpt-oss-20b & \cnd{max\_k\_shown} & 909 & 40.3 & 40.0 & 0.91 & 0.0 & 70.6 & 29.4 & 0.0 & 55.2 & 14.0 \\
  gpt-oss-20b & \cnd{min\_k\_shown} & 909 & 64.2 & 64.0 & 1.90 & 8.1 & 11.8 & 67.2 & 12.9 & 26.2 & 9.0 \\
  gpt-oss-20b & \cnd{min\_k\_shown\_fewer\_ok} & 909 & 39.3 & 38.9 & 1.14 & 4.4 & 58.7 & 29.8 & 7.0 & 49.7 & 11.4 \\
  gpt-oss-20b & \cnd{min\_k\_enforced} & 908 & 71.8 & 71.5 & 2.13 & 0.2 & 0.1 & 87.6 & 12.1 & 27.2 & 7.3 \\
  gpt-oss-20b & \cnd{min\_k\_escape} & 907 & 40.6 & 39.9 & 1.21 & 0.0 & 0.0 & 88.4 & 11.6 & 53.8 & 8.7 \\


==> generated/app_rq4_rows.tex <==
  job-ad skills & +1.54 [+0.83, +2.30] & +22.9 [+18.5, +27.4] \\
  job-ad knowledge & +0.76 [$-$0.26, +1.79] & +24.4 [+21.5, +27.3] \\


==> generated/app_sorting_per_model_rows.tex <==
  Qwen3.5-0.8B & \cnd{none} & 30.9 & 1.1 & 13.8 & 54.2 \\
  Qwen3.5-0.8B & \cnd{min\_k\_shown} & 24.9 & 0.3 & 7.4 & 67.4 \\
  Qwen3.5-0.8B & \cnd{min\_k\_shown\_fewer\_ok} & 34.0 & 0.4 & 16.5 & 49.1 \\
  Qwen3.5-0.8B & \cnd{max\_k\_shown} & 29.3 & 0.2 & 13.0 & 57.5 \\
  Qwen3.5-0.8B & \cnd{min\_k\_enforced} & 91.9 & 3.3 & 4.1 & 0.8 \\
  Qwen3.5-2B & \cnd{none} & 55.1 & 0.0 & 44.8 & 0.1 \\
  Qwen3.5-2B & \cnd{min\_k\_shown} & 60.4 & 0.0 & 39.4 & 0.2 \\
  Qwen3.5-2B & \cnd{min\_k\_shown\_fewer\_ok} & 46.9 & 0.0 & 52.5 & 0.7 \\
  Qwen3.5-2B & \cnd{max\_k\_shown} & 55.7 & 0.0 & 44.2 & 0.1 \\
  Qwen3.5-2B & \cnd{min\_k\_enforced} & 94.5 & 1.1 & 4.4 & 0.0 \\
  Qwen3.5-9B & \cnd{none} & 26.3 & 0.0 & 73.7 & 0.0 \\
  Qwen3.5-9B & \cnd{min\_k\_shown} & 44.8 & 0.0 & 55.1 & 0.1 \\
  Qwen3.5-9B & \cnd{min\_k\_shown\_fewer\_ok} & 18.0 & 0.0 & 82.0 & 0.0 \\
  Qwen3.5-9B & \cnd{max\_k\_shown} & 28.9 & 0.0 & 71.1 & 0.0 \\
  Qwen3.5-9B & \cnd{min\_k\_enforced} & 92.7 & 2.2 & 4.8 & 0.2 \\
  Qwen3.5-27B & \cnd{none} & 23.1 & 0.0 & 76.9 & 0.0 \\
  Qwen3.5-27B & \cnd{min\_k\_shown} & 60.9 & 0.0 & 36.6 & 2.4 \\
  Qwen3.5-27B & \cnd{min\_k\_shown\_fewer\_ok} & 42.2 & 0.1 & 56.1 & 1.5 \\
  Qwen3.5-27B & \cnd{max\_k\_shown} & 26.4 & 0.0 & 73.6 & 0.0 \\
  Qwen3.5-27B & \cnd{min\_k\_enforced} & 91.6 & 2.2 & 6.2 & 0.0 \\
  Gemma 4 31B & \cnd{none} & 14.4 & 0.0 & 85.6 & 0.0 \\
  Gemma 4 31B & \cnd{min\_k\_shown} & 62.5 & 18.5 & 15.1 & 4.0 \\
  Gemma 4 31B & \cnd{min\_k\_shown\_fewer\_ok} & 16.0 & 0.0 & 84.0 & 0.0 \\
  Gemma 4 31B & \cnd{max\_k\_shown} & 13.6 & 0.0 & 86.4 & 0.0 \\
  Gemma 4 31B & \cnd{min\_k\_enforced} & 85.6 & 8.0 & 6.4 & 0.0 \\
  Olmo 3.1 32B & \cnd{none} & 42.2 & 1.5 & 55.3 & 0.9 \\
  Olmo 3.1 32B & \cnd{min\_k\_shown} & 57.8 & 9.5 & 31.5 & 1.3 \\
  Olmo 3.1 32B & \cnd{min\_k\_shown\_fewer\_ok} & 18.7 & 6.9 & 71.5 & 2.9 \\
  Olmo 3.1 32B & \cnd{max\_k\_shown} & 45.0 & 1.7 & 52.5 & 0.9 \\
  Olmo 3.1 32B & \cnd{min\_k\_enforced} & 95.6 & 4.4 & 0.0 & 0.0 \\
  Ministral 3 14B & \cnd{none} & 50.2 & 0.0 & 49.8 & 0.0 \\
  Ministral 3 14B & \cnd{min\_k\_shown} & 67.7 & 14.1 & 18.3 & 0.0 \\
  Ministral 3 14B & \cnd{min\_k\_shown\_fewer\_ok} & 32.7 & 7.6 & 59.7 & 0.0 \\
  Ministral 3 14B & \cnd{max\_k\_shown} & 46.5 & 0.0 & 53.5 & 0.0 \\
  Ministral 3 14B & \cnd{min\_k\_enforced} & 97.2 & 2.0 & 0.4 & 0.3 \\
  gpt-oss-20b & \cnd{none} & 33.9 & 0.0 & 66.1 & 0.0 \\
  gpt-oss-20b & \cnd{min\_k\_shown} & 64.2 & 2.5 & 25.1 & 8.1 \\
  gpt-oss-20b & \cnd{min\_k\_shown\_fewer\_ok} & 39.3 & 0.7 & 55.7 & 4.4 \\
  gpt-oss-20b & \cnd{max\_k\_shown} & 40.3 & 0.0 & 59.7 & 0.0 \\
  gpt-oss-20b & \cnd{min\_k\_enforced} & 71.8 & 9.0 & 18.9 & 0.2 \\


==> generated/app_wordings_rows.tex <==
  \cnd{prose\_up\_to\_k} & up\_to\_1 & $-$0.85 [$-$1.02, $-$0.69] & 45.2 \\
  \cnd{prose\_up\_to\_k} & up\_to\_2 & $-$0.79 [$-$0.97, $-$0.61] & 42.4 \\
  \cnd{prose\_up\_to\_k} & up\_to\_3 & $-$0.61 [$-$0.77, $-$0.45] & 40.2 \\
  \cnd{prose\_up\_to\_k} & up\_to\_4 & $-$0.84 [$-$1.02, $-$0.67] & 45.9 \\
  \cnd{prose\_up\_to\_k} & up\_to\_5 & $-$0.72 [$-$0.89, $-$0.56] & 40.0 \\
  \cnd{prose\_exactly\_k} & exactly\_1 & $-$0.64 [$-$0.81, $-$0.47] & 59.7 \\
  \cnd{prose\_exactly\_k} & exactly\_2 & $-$0.51 [$-$0.68, $-$0.33] & 53.7 \\
  \cnd{prose\_exactly\_k} & exactly\_3 & $-$0.43 [$-$0.61, $-$0.25] & 51.0 \\
  \cnd{prose\_exactly\_k} & exactly\_4 & $-$0.71 [$-$0.89, $-$0.52] & 44.2 \\
  \cnd{prose\_exactly\_k} & exactly\_5 & $-$1.02 [$-$1.19, $-$0.84] & 45.8 \\


==> generated/tab_fill_main_rows.tex <==
  \cnd{none} & 18109 & 5.5 & 64.6 & 29.8 \\
  \cnd{max\_k\_shown} & 14697 & 5.7 & 66.3 & 27.9 \\
  \cnd{min\_k\_shown} & 22665 & 7.5 & 62.9 & 29.5 \\
  \cnd{min\_k\_shown\_fewer\_ok} & 13343 & 6.3 & 72.0 & 21.6 \\
  \cnd{min\_k\_enforced} & 26193 & 9.6 & 79.6 & 9.9 \\
  \cnd{min\_k\_escape} & 15198 & 9.8 & 82.4 & 7.2 \\

